Reinforcement Learning-based Knowledge Graph Reasoning for Explainable Fact-checking

Fact-checking is a crucial task as it ensures the prevention of misinformation. However, manual fact-checking cannot keep up with the rate at which false information is generated and disseminated online. Automated fact-checking by machines is significantly quicker than by humans. But for better trust and transparency of these automated systems, explainability in the fact-checking process is necessary. Fact-checking often entails contrasting a factual assertion with a body of knowledge for such explanations. An effective way of representing knowledge is the Knowledge Graph (KG). There have been sufficient works proposed related to fact-checking with the usage of KG but not much focus is given to the application of reinforcement learning (RL) in such cases. To mitigate this gap, we propose an RL-based KG reasoning approach for explainable fact-checking. Extensive experiments on FB15K-277 and NELL-995 datasets reveal that reasoning over a KG is an effective way of producing human-readable explanations in the form of paths and classifications for fact claims. The RL reasoning agent computes a path that either proves or disproves a factual claim, but does not provide a verdict itself. A verdict is reached by a voting mechanism that utilizes paths produced by the agent. These paths can be presented to human readers so that they themselves can decide whether or not the provided evidence is convincing or not. This work will encourage works in this direction for incorporating RL for explainable fact-checking as it increases trustworthiness by providing a human-in-the-loop approach.

==> dataset.tex <==
\section{Dataset}
    \begin{table}[h!]
\centering
\caption{Datasets}\label{Tbl:datatable}
\begin{tabular}{|l|c|c|c|}
\hline
Dataset   & \#Ent & \#Rel & \#Fact  \\ \hline
FB15k-237 & 14,505                        & 237   & 272,115 \\ \hline
NELL-995  & 75,492                        & 200   & 154,213 \\ \hline
\end{tabular}
\label{table:KGstats}
\end{table}
Table \ref{table:KGstats}: Statistics of the datasets. \#Ent denotes the number of unique entities and \#Rel denotes the number of relations.

The experiments are conducted on two benchmark datasets: NELL-995 \cite{Xiong2017} and FB15K-237 \cite{Toutanova2015}. The details of the two datasets are described in Table \ref{table:KGstats}. For each triple (h, r, t), both datasets contain the inverse triple (h, $r^{-1}$, t) such that the agent can step backward in KGs. For each reasoning task with a query relation $r_q$, all the triples with $r_q$ or $r_q^{-1}$ are removed from the KG and split into train and test samples. NELL-995 is generated from the 995th iteration of the NELL system \cite{Carlson2010} by selecting the triples with the top 200 most frequent relations. FB15K-237's facts are created from FB15K \cite{Bordes2013} with redundant relations removed.


    

==> preliminaries.tex <==
\section{Preliminaries}\label{chp:Prelim}





\begin{comment}
\subsection{Rundown, case study?}
\TODO{Bring everything discussed thus fur into an example run of the architecture}
\subsubsection{What happens in a training episode}
\subsubsection{What happens in a testing episode}
\TODO{Introduce BEAM search here? Add a section into preliminaries, Introduce voting here?}
\end{comment}

==> results.tex <==
\section{Results}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


